Breaking Boundaries: Distributed Domain Decomposition with Scalable Physics-Informed Neural PDE Solvers

Mosaic Flow is a novel domain decomposition method designed to scale physics-informed neural PDE solvers to large domains. Its unique approach leverages pre-trained networks on small domains to solve partial differential equations on large domains purely through inference, resulting in high reusability. This paper presents an end-to-end parallelization of Mosaic Flow, combining data parallel training and domain parallelism for inference on large-scale problems. By optimizing the network architecture and data parallel training, we significantly reduce the training time for learning the Laplacian operator to minutes on 32 GPUs. Moreover, our distributed domain decomposition algorithm enables scalable inferences for solving the Laplace equation on domains 4096 times larger than the training domain, demonstrating strong scaling while maintaining accuracy on 32 GPUs. The reusability of Mosaic Flow, combined with the improved performance achieved through the distributed-memory algorithms, makes it a promising tool for modeling complex physical phenomena and accelerating scientific discovery.

==> alg/MFAlg.tex <==
\begin{algorithm}[h]
\centering
\begin{algorithmic}
%\Function{MosaicFlows}{$m$, $\Omega$}
\State $m$ is a pretrained GFNet
\State $\Omega$ is the global domain
\State Construct $S$, a list of overlapping subdomains of $\Omega$
\While{not converged}
    \For{$s$ in $S$}
        \State $\hat{g}$ is the boundary of $s$
        \State $\textbf{x}_{center}$ is the coordinates of the center lines of $s$
        \State $b_{center}$ = $m(\hat{g},
 \textbf{x}_{center})$
        \State $\Omega(x_{center})$ = $b_{center}$
    \EndFor
\EndWhile
%\EndFunction
\end{algorithmic}
\caption{Mosaic Flows}
\label{alg:mf}
\end{algorithm}

==> alg/mfpred-new.tex <==
\begin{verbatim}
Function iterativeSolve()
  bc = boundary of overall domain
  genome_levels = []
  level = 0
  while(there are areas of the domain uncovered by a genome):
    genome_levels[level] = generate genomes along bc
    bc = center-line of genome_levels[level]
    level++
  for genomes in genome_levels:
      old_solution = solve genomes
  while(!converged):
    for genomes in genome_levels:
      new_solution = solve genomes
    if(new_solution - old_solution < epsilon):
      converged = true
\end{verbatim}


==> figures/communication.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.4,xscale=0.4]
%uncomment if require: \path (0,599); %set diagram left start at 0, and has height of 599

%Shape: Rectangle [id:dp7466857946937417] 
\draw  [line width=0.75]  (0,0) -- (240,0) -- (240,240) -- (0,240) -- cycle ;
%Shape: Rectangle [id:dp405403827745908] 
\draw  [line width=0.75]  (240,0) -- (480,0) -- (480,240) -- (240,240) -- cycle ;
%Shape: Rectangle [id:dp7834300515143129] 
\draw  [line width=0.75]  (240,240) -- (480,240) -- (480,480) -- (240,480) -- cycle ;
%Shape: Rectangle [id:dp05765992845564227] 
\draw  [line width=0.75]  (0,240) -- (240,240) -- (240,480) -- (0,480) -- cycle ;
%Straight Lines [id:da028731971157249125] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (260,240) -- (260,300) ;
%Straight Lines [id:da6740580103179354] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (300,240) -- (300,300) ;
%Straight Lines [id:da6858891788092851] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,200) -- (239.5,200) ;
%Straight Lines [id:da5775722331140554] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,220) -- (240,220) ;
%Straight Lines [id:da9253380982177264] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (300,260) -- (240,260) ;
%Straight Lines [id:da3060605297788954] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (300,280) -- (240,280) ;
%Straight Lines [id:da6111261749366133] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (0,240) -- (240,240) ;
%Straight Lines [id:da08382548538968915] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (280,240) -- (280,300) ;
%Straight Lines [id:da009911080987882848] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (300,300) -- (240,300) ;
%Straight Lines [id:da9425586540552153] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,180) -- (240,180) ;
%Straight Lines [id:da8781122985196201] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (240,0) -- (240,240) ;
%Straight Lines [id:da5294155950216717] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (0,260) -- (240,260) ;
%Straight Lines [id:da4029224308038022] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (0,280) -- (240,280) ;
%Straight Lines [id:da15526479351952593] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (0,300) -- (240,300) ;
%Straight Lines [id:da028287240503814592] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (220,240) -- (220,300) ;
%Straight Lines [id:da027043747092785342] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (200,240) -- (200,300) ;
%Straight Lines [id:da637285132120063] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (20,240) -- (20,300) ;
%Straight Lines [id:da2807949787688784] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (40,240) -- (40,300) ;
%Straight Lines [id:da3260110772813276] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (60,240) -- (60,300) ;
%Straight Lines [id:da18742443809878617] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (80,240) -- (80,300) ;
%Straight Lines [id:da32234522741103455] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (100,240) -- (100,300) ;
%Straight Lines [id:da48811501867837515] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (120,240) -- (120,300) ;
%Straight Lines [id:da11873606289234506] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (140,240) -- (140,300) ;
%Straight Lines [id:da8438603448118946] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (160,240) -- (160,300) ;
%Straight Lines [id:da6487690305056875] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (180,240) -- (180,300) ;
%Straight Lines [id:da9032308754051432] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (240,240) -- (240,300) ;
%Straight Lines [id:da2612348096375172] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (260,0) -- (260,240) ;
%Straight Lines [id:da035472754829420694] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (280,0) -- (280,240) ;
%Straight Lines [id:da24912571638463943] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,0) -- (300,240) ;
%Straight Lines [id:da7207289947835331] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,20) -- (240,20) ;
%Straight Lines [id:da8751277985199561] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,40) -- (240,40) ;
%Straight Lines [id:da8222612889656613] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,60) -- (240,60) ;
%Straight Lines [id:da48246046542443155] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,80) -- (240,80) ;
%Straight Lines [id:da051487129625104044] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,100) -- (240,100) ;
%Straight Lines [id:da38916743048170743] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,120) -- (240,120) ;
%Straight Lines [id:da06674538366586291] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,140) -- (240,140) ;
%Straight Lines [id:da18788888940048198] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (300,160) -- (240,160) ;
%Straight Lines [id:da32423232513801725] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (300,240) -- (240,240) ;
%Straight Lines [id:da16789943708368282] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (320,0) -- (320,480) ;
%Straight Lines [id:da6245185110632345] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (400,0) -- (400,480) ;
%Straight Lines [id:da2386641247289174] 
\draw [line width=0.75]  [dash pattern={on 4.5pt off 4.5pt}]  (160,0) -- (160,480) ;
%Straight Lines [id:da6153554825545497] 
\draw [line width=0.75]  [dash pattern={on 4.5pt off 4.5pt}]  (80,-1) -- (80,479) ;
%Straight Lines [id:da8368155721486954] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (0,400) -- (480,400) ;
%Straight Lines [id:da5442711806721339] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (0,320) -- (480,320) ;
%Straight Lines [id:da5069261745561398] 
\draw [line width=0.75]  [dash pattern={on 4.5pt off 4.5pt}]  (0,160) -- (480,160) ;
%Straight Lines [id:da2868731960149593] 
\draw [line width=0.75]  [dash pattern={on 4.5pt off 4.5pt}]  (0,80) -- (480,80) ;




\end{tikzpicture}

==> figures/distribution.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.4,xscale=0.4]
%uncomment if require: \path (0,599); %set diagram left start at 0, and has height of 599

%Shape: Rectangle [id:dp7466857946937417] 
\draw  [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=0.3 ][line width=0.75]  (0,0) -- (300,0) -- (300,300) -- (0,300) -- cycle ;
%Shape: Rectangle [id:dp405403827745908] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ][line width=0.75]  (180,0) -- (480,0) -- (480,300) -- (180,300) -- cycle ;
%Shape: Rectangle [id:dp7834300515143129] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=0.3 ][line width=0.75]  (180,180) -- (480,180) -- (480,480) -- (180,480) -- cycle ;
%Shape: Rectangle [id:dp05765992845564227] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.3 ][line width=0.75]  (0,180) -- (300,180) -- (300,480) -- (0,480) -- cycle ;
%Straight Lines [id:da43062596579473844] 
\draw    (0,300) -- (480,300) ;
%Straight Lines [id:da8906476408484476] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (0,240) -- (480,240) ;
%Straight Lines [id:da32044229351730436] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (240,0) -- (240,480) ;
\end{tikzpicture}

==> figures/distribution/basicGenomePlacement.tex <==



%uncomment if require: \path (0,676); %set diagram left start at 0, and has height of 676

%Straight Lines [id:da478216383517978] 
\draw    (260,96.33) -- (260,576.33) ;
%Straight Lines [id:da8424164825141109] 
\draw    (100,256.33) -- (580,256.33) ;
%Shape: Brace [id:dp11156936795192562] 
\draw   (103,582.33) .. controls (103.01,587) and (105.35,589.32) .. (110.02,589.31) -- (331.02,588.62) .. controls (337.69,588.6) and (341.03,590.92) .. (341.04,595.59) .. controls (341.03,590.92) and (344.35,588.58) .. (351.02,588.55)(348.02,588.56) -- (572.02,587.86) .. controls (576.69,587.85) and (579.01,585.51) .. (579,580.84) ;
%Shape: Brace [id:dp8307714609150132] 
\draw   (93,95.83) .. controls (88.33,95.78) and (85.97,98.08) .. (85.91,102.74) -- (85.12,165.75) .. controls (85.04,172.42) and (82.67,175.72) .. (78,175.66) .. controls (82.67,175.72) and (84.96,179.08) .. (84.87,185.74)(84.91,182.74) -- (84.08,248.75) .. controls (84.02,253.42) and (86.32,255.78) .. (90.99,255.83) ;
%Shape: Brace [id:dp21244883456131802] 
\draw   (299.83,92.33) .. controls (299.76,87.66) and (297.39,85.37) .. (292.72,85.45) -- (290.05,85.5) .. controls (283.38,85.61) and (280.01,83.33) .. (279.94,78.66) .. controls (280.01,83.33) and (276.72,85.72) .. (270.06,85.83)(273.06,85.78) -- (267.05,85.88) .. controls (262.38,85.96) and (260.09,88.33) .. (260.17,93) ;
%Shape: Rectangle [id:dp6715669972579279] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.3 ] (100,96.33) -- (300,96.33) -- (300,296.33) -- (100,296.33) -- cycle ;
%Shape: Rectangle [id:dp017929386870610298] 
\draw   (100,96.33) -- (580,96.33) -- (580,576.33) -- (100,576.33) -- cycle ;
%Straight Lines [id:da3334836932548193] 
\draw    (420,96.33) -- (420,576.33) ;
%Straight Lines [id:da9854483220521317] 
\draw    (100,416.33) -- (580,416.33) ;
%Shape: Rectangle [id:dp0428634452986596] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (220,216.33) -- (460,216.33) -- (460,456.33) -- (220,456.33) -- cycle ;
%Straight Lines [id:da2107886852303682] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (180,96.33) -- (180,576.33) ;
%Straight Lines [id:da0738277331949333] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (340,96.33) -- (340,576.33) ;
%Straight Lines [id:da4302118271924784] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (500,96.33) -- (500,576.33) ;
%Straight Lines [id:da9263736049013407] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (100,496.33) -- (580,496.33) ;
%Straight Lines [id:da6004341545822498] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (100,336.33) -- (580,336.33) ;
%Straight Lines [id:da5798168635091161] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (100,176.33) -- (580,176.33) ;
%Shape: Brace [id:dp6771879493018242] 
\draw   (179.5,94.75) .. controls (179.55,90.08) and (177.24,87.73) .. (172.57,87.68) -- (152.21,87.48) .. controls (145.54,87.42) and (142.23,85.06) .. (142.28,80.39) .. controls (142.23,85.06) and (138.88,87.36) .. (132.22,87.29)(135.22,87.32) -- (109.23,87.06) .. controls (104.57,87.01) and (102.22,89.32) .. (102.17,93.99) ;

% Text Node
\draw (335,600.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle N$};
% Text Node
\draw (41,152.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{N}{\sqrt{P}}$};
% Text Node
\draw (251,42) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{d-1}{d} g$};
% Text Node
\draw (138.5,59) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle g$};


==> figures/distribution/communication.tex <==
%Straight Lines [id:da6162685268257866] 
\draw    (240,80) -- (240,560) ;
%Straight Lines [id:da023455363996819578] 
\draw    (80,240) -- (560,240) ;
%Shape: Rectangle [id:dp8346137522146437] 
\draw   (80,80) -- (560,80) -- (560,560) -- (80,560) -- cycle ;
%Straight Lines [id:da16066608609841904] 
\draw    (400,80) -- (400,560) ;
%Straight Lines [id:da04778193715042689] 
\draw    (80,400) -- (560,400) ;
%Straight Lines [id:da23224590722978355] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (160,80) -- (160,560) ;
%Straight Lines [id:da7128420296664937] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (320,80) -- (320,560) ;
%Straight Lines [id:da6260705205182369] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (480,80) -- (480,560) ;
%Straight Lines [id:da5748010301556037] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (80,480) -- (560,480) ;
%Straight Lines [id:da900436381756488] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (80,320) -- (560,320) ;
%Straight Lines [id:da18831041714645913] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,220) -- (240,220) ;
%Straight Lines [id:da94973447530377] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,220) -- (440,220) ;
%Straight Lines [id:da015167399262596915] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,420) -- (440,420) ;
%Straight Lines [id:da47126201183224636] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,420) -- (240,420) ;
%Straight Lines [id:da8425790280681535] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (220,440) -- (220,400) ;
%Straight Lines [id:da7379697992658167] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (220,240) -- (220,200) ;
%Straight Lines [id:da7241313299740013] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (420,240) -- (420,200) ;
%Straight Lines [id:da8285833813959607] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (420,440) -- (420,400) ;
%Straight Lines [id:da5926765623497363] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,420) -- (400,420) ;
%Straight Lines [id:da5447765498288584] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,220) -- (400,220) ;
%Straight Lines [id:da8298165161514266] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (380,240) -- (380,200) ;
%Straight Lines [id:da6621772019029837] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (360,240) -- (360,200) ;
%Straight Lines [id:da05966754764830706] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (340,240) -- (340,200) ;
%Straight Lines [id:da2969466833777583] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (320,240) -- (320,200) ;
%Straight Lines [id:da085923787192282] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (300,240) -- (300,200) ;
%Straight Lines [id:da42626404184501476] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (280,240) -- (280,200) ;
%Straight Lines [id:da21423475739415854] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (260,240) -- (260,200) ;
%Straight Lines [id:da14853917704239028] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (240,240) -- (240,200) ;
%Straight Lines [id:da6417029244132368] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,240) -- (400,200) ;
%Straight Lines [id:da011377914004446099] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (380,440) -- (380,400) ;
%Straight Lines [id:da9690470010545951] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (360,440) -- (360,400) ;
%Straight Lines [id:da8683990411041436] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (340,440) -- (340,400) ;
%Straight Lines [id:da8549303992198563] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (320,440) -- (320,400) ;
%Straight Lines [id:da4676822960206348] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (300,440) -- (300,400) ;
%Straight Lines [id:da5573831963525744] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (280,440) -- (280,400) ;
%Straight Lines [id:da8361337403876827] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (260,440) -- (260,400) ;
%Straight Lines [id:da1958063145212252] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (240,440) -- (240,400) ;
%Straight Lines [id:da149236173413819] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,440) -- (400,400) ;
%Straight Lines [id:da26436217477017854] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,440) -- (440,440) ;
%Straight Lines [id:da07656963268391936] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,440) -- (240,440) ;
%Straight Lines [id:da5869192443419231] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,440) -- (400,440) ;
%Straight Lines [id:da33120914797144496] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,400) -- (400,400) ;
%Straight Lines [id:da34920155470741876] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,240) -- (400,240) ;
%Straight Lines [id:da562028478782139] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,200) -- (400,200) ;
%Straight Lines [id:da5317909894788229] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,400) -- (440,400) ;
%Straight Lines [id:da935919190358022] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,240) -- (240,240) ;
%Straight Lines [id:da5005572205335993] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,200) -- (240,200) ;
%Straight Lines [id:da2801252008906394] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,200) -- (440,200) ;
%Straight Lines [id:da5524730966016305] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (400,240) -- (440,240) ;
%Straight Lines [id:da9004513913315522] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,400) -- (400,240) ;
%Straight Lines [id:da0824080184595799] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (420,400) -- (420,240) ;
%Straight Lines [id:da7026399492291229] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (440,400) -- (440,240) ;
%Straight Lines [id:da15800200757347826] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (220,400) -- (220,240) ;
%Straight Lines [id:da002343713135929404] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (240,400) -- (240,240) ;
%Straight Lines [id:da20175229094248093] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,400) -- (200,240) ;
%Straight Lines [id:da20223145422096955] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,440) -- (200,400) ;
%Straight Lines [id:da2355791916763672] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (440,440) -- (440,400) ;
%Straight Lines [id:da028660024254836713] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (440,240) -- (440,200) ;
%Straight Lines [id:da45599339088631585] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,240) -- (200,200) ;
%Straight Lines [id:da15568515709674502] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,260) -- (240,260) ;
%Straight Lines [id:da705512232894463] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,300) -- (240,300) ;
%Straight Lines [id:da08596497579185769] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,320) -- (240,320) ;
%Straight Lines [id:da9674622979526057] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,280) -- (240,280) ;
%Straight Lines [id:da651311388126611] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,340) -- (240,340) ;
%Straight Lines [id:da6238882678777522] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,380) -- (240,380) ;
%Straight Lines [id:da3470328246718579] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (200,360) -- (240,360) ;
%Straight Lines [id:da8295882546355515] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (200,400) -- (240,400) ;
%Straight Lines [id:da22354106768258797] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,260) -- (440,260) ;
%Straight Lines [id:da1411200684732712] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,300) -- (440,300) ;
%Straight Lines [id:da6768477784287865] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,280) -- (440,280) ;
%Straight Lines [id:da338168923867999] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,340) -- (440,340) ;
%Straight Lines [id:da9526348340198891] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,380) -- (440,380) ;
%Straight Lines [id:da447953205498381] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,360) -- (440,360) ;
%Straight Lines [id:da12082284526783749] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (400,320) -- (440,320) ;
%Shape: Brace [id:dp2024663892585148] 
\draw   (197,201.5) .. controls (192.33,201.63) and (190.06,204.02) .. (190.19,208.69) -- (190.26,211.11) .. controls (190.44,217.78) and (188.2,221.17) .. (183.53,221.3) .. controls (188.2,221.17) and (190.62,224.44) .. (190.8,231.1)(190.72,228.1) -- (190.81,231.69) .. controls (190.94,236.36) and (193.33,238.63) .. (198,238.5) ;
%Shape: Brace [id:dp21499376525137714] 
\draw   (243,243.5) .. controls (243.03,248.17) and (245.38,250.48) .. (250.05,250.45) -- (280.14,250.26) .. controls (286.81,250.22) and (290.15,252.53) .. (290.18,257.2) .. controls (290.15,252.53) and (293.47,250.18) .. (300.14,250.13)(297.14,250.15) -- (390.05,249.55) .. controls (394.72,249.52) and (397.03,247.18) .. (397,242.51) ;
%Shape: Brace [id:dp22654421074369147] 
\draw   (82,565.33) .. controls (82.01,570) and (84.35,572.32) .. (89.02,572.31) -- (310.02,571.62) .. controls (316.69,571.6) and (320.03,573.92) .. (320.04,578.59) .. controls (320.03,573.92) and (323.35,571.58) .. (330.02,571.55)(327.02,571.56) -- (551.02,570.86) .. controls (555.69,570.85) and (558.01,568.51) .. (558,563.84) ;
%Straight Lines [id:da23589386111314603] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (80,160) -- (560,160) ;

% Text Node
\draw (106,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{d-1}{d} g$};
% Text Node
\draw (271,261.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{N}{\sqrt{P}}$};
% Text Node
\draw (314,583.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle N$};


==> figures/distribution/subdomainDistribution.tex <==

%Straight Lines [id:da11241579554358028] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (240,80) -- (240,560) ;
%Straight Lines [id:da5951319796167513] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (80,240) -- (560,240) ;
%Shape: Brace [id:dp22364137873376344] 
\draw   (83,566) .. controls (83.01,570.67) and (85.35,572.99) .. (90.02,572.98) -- (311.02,572.28) .. controls (317.69,572.26) and (321.03,574.58) .. (321.04,579.25) .. controls (321.03,574.58) and (324.35,572.24) .. (331.02,572.22)(328.02,572.23) -- (552.02,571.53) .. controls (556.69,571.51) and (559.01,569.17) .. (559,564.5) ;
%Shape: Brace [id:dp8554289266121411] 
\draw   (73,79.5) .. controls (68.33,79.44) and (65.97,81.74) .. (65.91,86.41) -- (65.12,149.41) .. controls (65.04,156.08) and (62.67,159.38) .. (58,159.32) .. controls (62.67,159.38) and (64.96,162.74) .. (64.87,169.41)(64.91,166.41) -- (64.08,232.41) .. controls (64.02,237.08) and (66.32,239.44) .. (70.99,239.5) ;
%Shape: Brace [id:dp7512867375841854] 
\draw   (279.83,76) .. controls (279.76,71.33) and (277.39,69.04) .. (272.72,69.12) -- (270.05,69.16) .. controls (263.38,69.27) and (260.01,67) .. (259.94,62.33) .. controls (260.01,67) and (256.72,69.39) .. (250.06,69.5)(253.06,69.45) -- (247.05,69.55) .. controls (242.38,69.63) and (240.09,72) .. (240.17,76.66) ;
%Shape: Rectangle [id:dp356267641686693] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.3 ] (80,80) -- (280,80) -- (280,280) -- (80,280) -- cycle ;
%Shape: Rectangle [id:dp39504329433129737] 
\draw   (80,80) -- (560,80) -- (560,560) -- (80,560) -- cycle ;
%Straight Lines [id:da7956963317593404] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (400,80) -- (400,560) ;
%Straight Lines [id:da7293776826005054] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (80,400) -- (560,400) ;
%Shape: Rectangle [id:dp4965530776514988] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (200,200) -- (440,200) -- (440,440) -- (200,440) -- cycle ;

% Text Node
\draw (315,584.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {N};
% Text Node
\draw (21,136) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{N}{\sqrt{P}}$};
% Text Node
\draw (169,161.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle P_{0}$};
% Text Node
\draw (231,25.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \frac{d-1}{d} g$};
% Text Node
\draw (312,310.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle P_{4}$};


==> src/faq.tex <==
\section{Frequency Asked Questions}

There are several common questions that we received about this work, which we respond to here:

\begin{enumerate}
    \item \textbf{} Is okay
    \item \textbf{} IDK
    \item \textbf{Can this method be extended to other PDEs?} Yes, but it is not fully generic. The Alternating Schwarz Method was originally developed as a tool for general elliptic PDEs on irregular domains. However, in practice, \mf has been able to approximate solutions to more complicated PDEs, such as Laminar flow governed by the Navier-Stokes equations \cite{wang2022mosaic}, which is non-linear and hyperbolic. However, to our knowledge, there is no motivating theory for convergence in this case. There are some PDEs that \mf will may fail to solve in general. For instance, it has been shown that ASM can fail to converge on problems of Helmholtz type \cite{gander2006optimized}.
\end{enumerate}

==> src/mfpred.tex <==
\section{New MF Predictor -- \update{Zitong leads}}

\begin{algorithm} [htbp]
\input{alg/mfpred-new.tex}
\caption{New MF Predictor algorithm \update{The algorithm will generate genomes for steps 1-3 in figure \ref{fig:mfpred} but not step 4 since after the first 3 steps, there are no areas of the domain that’s not covered by a genome.}}
\label{alg:mfprednew}
\end{algorithm}

\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.45]{figures/MFPred.png}
	\caption{MF Predictor -- new vs. old
	\label{fig:mfpred}}
\end{figure}
